CheckSync: Using Runtime-Integrated Checkpoints to Achieve High Availability}

CheckSync provides applications with high availability via runtime-integrated checkpointing. This allows CheckSync to take checkpoints of a process running in a memory-managed language (Go, for now), which can be resumed on another machine after a failure. CheckSync uses the runtime to checkpoint only the process' live memory, doing without requiring significant changes to applications. CheckSync maintains the ease of use provided by virtual machines for the applications it supports without requiring that an entire virtual machine image be snapshotted. Because CheckSync captures only the memory used by an application, it produces checkpoints that are smaller (by an order of magnitude) than virtual machine snapshots if the memory footprint of the application is relatively small compared to the state of the rest of the operating system. Additionally, when running go-cache, a popular in-memory key/value store, CheckSync reduces throughput by only 12% compared to the 78% throughput loss when using go-cache's snapshot functionality, the 45% loss when using CRIU, and the 68% loss when using virtual machine live migration.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}
CheckSync seeks to address the weaknesses of existing techniques for providing high availability to mission critical applications. The class of applications CheckSync seeks to support are components of larger systems that are necessary for the larger system to function. We characterize these applications as running in-memory, although CheckSync does replicate open files as well. These applications require good performance, and often use parallelism to achieve this. Additionally, these applications must use the network to make themselves available to other components of the larger system.


Existing solutions do a poor job of providing high availability to these services. Replicated state machines are both hard to use and hamper performance. Virtual machines address one of these concerns, but are still slow. CheckSync strikes a middle ground by targeting a specific class of applications, allowing it to deliver ease of use and high performance.
